How to design, and tune, a computed torque controller: An introduction and a Matlab example

This note briefly introduces the computed torque control method for trajectory tracking. The method is applicable to fully actuated robots, i.e, those whose inverse dynamics can be solved for any feasible acceleration. This includes many systems, like robot arms or hands, or any tree-like mechanism with all its joints actuated. Using simple explanations, we see how such a controller can be obtained using feedback linearization, and how its gains can be tuned to satisfy a desired settling time for the error signal. We end up discussing the advantages and shortcomings of the controller. A companion Matlab script can be downloaded from https://bit.ly/3QShxYi that implements and tests the controller on a simple actuated pendulum.

==> Makefile <==

########################################################################
# 		 	Commands and variables
########################################################################

#----------------------------------------------------
# Set the main *.tex document name
#----------------------------------------------------
DOC = ctc

#----------------------------------------------------
# Choose paper format ('a4' or 'letter')
#----------------------------------------------------
PAPER = a4

#----------------------------------------------------
# Extensions of files to be cleaned
#----------------------------------------------------
EXT= *.aux *.toc *.log *.spl *.lot *.lof \
     *.ttt *.fff *.blg *.out *.dvi *.bbl \
     *.nlo *.idx *.ind *.ilg *.thm       \
     *-eps-converted-to.pdf *.bak *.tex~ \
     *.backup *.bak

#----------------------------------------------------
# Compilation commands
#
# In PS2PDF, changing 'prepress' to 'screen' 
# produces much smaller files 
#----------------------------------------------------

TEX = latex
PDFTEX = pdflatex
BIBTEX = bibtex
RM = rm -f

PS2PDF = gs -sOutputFile=$(DOC).pdf -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -r600 -dPDFSETTINGS=/prepress -dSubsetFonts=true -dMaxSubsetPct=100 -dEmbedAllFonts=true -dEncodeGrayImages=true -dEncodeColorImages=true

########################################################################
# 				Rules
########################################################################

pdf: $(DOC).tex 
	$(PDFTEX) --shell-escape $(DOC)
	$(BIBTEX) $(DOC)
	$(PDFTEX) --shell-escape $(DOC)
	$(PDFTEX) --shell-escape $(DOC)

fast: $(DOC).tex
	$(PDFTEX) --shell-escape $(DOC)

aux: $(DOC).tex 
	$(TEX) $(DOC).tex

bib: aux 
	$(BIBTEX) $(DOC)

dvi: aux bib  
	$(TEX) $(DOC).tex
	$(TEX) $(DOC).tex

final: 
	$(PDFTEX) $(DOC)
	$(PDFTEX) $(DOC)
	$(BIBTEX) $(DOC)
	$(PDFTEX) $(DOC)

clean: 
	$(RM) $(DOC).ps $(DOC)-*.ps
	$(RM) $(DOC).pdf
	$(RM) Makefile~
	$(RM) $(DOC).synctex.gz
	for i in $(EXT); do find . -name "$$i" -delete; done


